Geometric properties of solutions to the total variation denoising problem

This article studies the denoising performance of total variation (TV) image regularization. More precisely, we study geometrical properties of the solution to the so-called Rudin-Osher-Fatemi total variation denoising method. The first contribution of this paper is a precise mathematical definition of the "extended support" (associated to the noise-free image) of TV denoising. It is intuitively the region which is unstable and will suffer from the staircasing effect. We highlight in several practical cases, such as the indicator of convex sets, that this region can be determined explicitly. Our second and main contribution is a proof that the TV denoising method indeed restores an image which is exactly constant outside a small tube surrounding the extended support. The radius of this tube shrinks toward zero as the noise level vanishes, and are able to determine, in some cases, an upper bound on the convergence rate. For indicators of so-called "calibrable" sets (such as disks or properly eroded squares), this extended support matches the edges, so that discontinuities produced by TV denoising cluster tightly around the edges. In contrast, for indicators of more general shapes or for complicated images, this extended support can be larger. Beside these main results, our paper also proves several intermediate results about fine properties of TV regularization, in particular for indicators of calibrable and convex sets, which are of independent interest.

==> sections/sec-burger-osher.tex <==
% !TEX root = ../TV-Denoising.tex

\section{The Burger-Osher approach}
\label{sec-burger-osher}

\todo{We should remove this section and place a discussion in the introduction/our contributions section where we discuss the significance of the MNC: standard certificates give integral stability estimates, but the MNC will additionally provide structural estimates. }


\todo{The aim of this section is different from the rest of the paper. We study the bound on the total variation provided by Burger and Osher outside the tube. We show that this enables to bound the oscillation (but not the support of the gradient)
}
Let $u_0\in \LDD$.
Let $u_\lambda$ be a minimizer of (\ref{eq-rof}), with $\norm{ f -  u_0}_{L^2}\leq \delta$. Let $p\in \LDD$ be such that $v \in \partial J (u_0)$ and so, there exists $z\in \mathrm{L}^\infty(\RR^2, \RR^2)$ so that $v = -\divx z$, $(z, D u_0) = \abs{Du_0}$ and $\normi{z}\leq 1$. Let $T_r$ be a ring of width $r$ around the saturation points of $z_0$ so that $\abs{z(x)}<1- e_r$ with $e_r\in (0,1)$ for a.e. $x\in T_r^c$.


We first recall two results and their proofs from \cite{burger2004convergence}.


\begin{thm}\label{thm:burger}\cite{burger2004convergence}
$$
J(u_\lambda) - J(u_0) - \dotp{v}{u_\lambda-u_0}\leq \frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2}.
$$
\end{thm}
\begin{proof}
Let $d=  J(u_\lambda) -  J(u_0) - \dotp{v}{u_\lambda-u_0}$. Since $u^\lambda$ is a minimizer of (\ref{eq-rof}),
$$
\lambda J(u_\lambda) + \frac{1}{2}\norm{ u_\lambda - f}_{L^2}^2 \leq \lambda J(u_0) +  \frac{1}{2}\norm{ u_0 - f}_{L^2}^2\leq \lambda J(u_0) + \frac{\delta^2}{2}.$$
It follows that 
\begin{align*}
 \frac{1}{2}\norm{ u_\lambda - f}_{L^2}^2 +  \lambda d + \lambda \dotp{v}{u_\lambda - u_0} \leq \frac{\delta^2}{2}\\
\implies \frac{1}{2}\norm{ u_\lambda - f}_{L^2}^2 + \lambda d + \lambda \dotp{v}{ u_\lambda - f} + \lambda \dotp{v}{f -  u_0 } \leq \frac{\delta^2}{2}\\
\implies \frac{1}{2}\norm{ u_\lambda - f + \lambda v}_{L^2}^2 + \lambda d - \frac{\lambda^2 \norm{v}_{L^2}^2}{2} + \lambda \dotp{v}{f -  u_0 } \leq \frac{\delta^2}{2}.
\end{align*}
Therefore,
$$
d\leq \frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2} .
$$
\end{proof}




  
  We have the following result from \cite{burger2004convergence}, from which we may bound the height of the jumps of $u_\lambda$ outside $T_r$ in Theorem \ref{thm:jump_height}.



\begin{thm}\cite{burger2004convergence}\label{thm:burger_outside_tube}
For each $r>0$,
$$
(1-e_r)\int_{T_r^c} \abs{D u_\lambda}\leq  \frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2}.
$$
\end{thm}
\begin{proof}
\begin{align*}
&d:= J(u_\lambda) - J(u_0) - \dotp{v}{u_\lambda-u_0}\\
&= J(u_\lambda) - J(u_0) + \dotp{\divx z}{u_\lambda} -\dotp{\divx z }{u}\\
&= J(u_\lambda)  + \dotp{\divx z}{u_\lambda}\\
&= J(u_\lambda)  -\int ( z, D u_\lambda)\\
&= J(u_\lambda)  -\int_{T_r} ( z, D u_\lambda) -\int_{T_r^c} ( z, D u_\lambda)\\
&\geq J(u_\lambda)  -\int_{T_r}\abs{D u_\lambda} -e_r \int_{T_r^c} \abs{D u_\lambda}\\
&\geq (1-e_r) \int_{T_r^c} \abs{D u_\lambda}.
\end{align*}
The conclusion now follows by applying the upper bound on $d$ from Theorem \ref{thm:burger}.
\end{proof}



\begin{thm}\label{thm:jump_height}
Let $B$ be any connected subset of $T_r^c$. Then,
$$
\mathrm{ess}\sup_B u - \mathrm{ess}\inf_B u = \Oo \left(\frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2}\right).
$$
\end{thm}

\begin{proof}
Assume that $u$ is not constant a.e. on $B$. Let $F_t = \{ u> t \}$. Then,
$$
\mathrm{ess}\sup_B u = \sup_t \{ t: F_t \cap B \neq \emptyset \}, \qquad \mathrm{ess}\inf_B u = \sup \{ t: F_t\supseteq B \}.
$$ 
Let $s_2 := \mathrm{ess}\sup_B u$ and $s_1:= \mathrm{ess}\inf_B u$. Note that $s_2>s_1$ since $u$ is not constant a.e. on $B$. 


We first show that $\Hh^1(\partial^* F_{t} \cap T_r^c)>0$ for all $t\in (s_1,s_2)$:  
Recall from Section \ref{sec:prelim} that for each $t$, there exists $E_t$ and Jordan curves $\{J_{j}^{(t)}\}_{j=1}^K$ such that  $\partial^M E_t = \cup_{j=1}^{K}J_{j}^{(t)}$, $E_t = F_t$ (up to $\Hh^2$) and $\partial^M E_t = \partial^M F_t$ (up to $\Hh^1$). In particular, $\partial E_t$ is of class $\Cder{}$.
Note also that $\partial^M F_t = \partial^* F_t$ up to $\Hh^1$.


 Since $F_{s_1}\supseteq F_t \supseteq F_{s_2}$, it follows that $E_{s_1}\supseteq E_t \supseteq E_{s_2}$, $E_t\cap B \neq \emptyset$ and $E_t\not\supseteq B$. This implies that   $\Hh^1(\partial^M E_t \cap B) >0$  because $B$ is connected. Since $B\subseteq T_r^c$, we have that $\Hh^1(\partial^M E_t \cap T_r^c)>0$.


If $\Hh^1(\partial^M E_s\cap T_{r/2})= \Hh^1(\partial^* F_s\cap T_{r/2})=0$ for all $s\in (s_1,s_2)$, then by Proposition \ref{prop:curvature_viaBurger} and Theorem \ref{thm:burger_outside_tube}, there exists $C>0$ and $\la_0>0$ such that
$$
 s_2-s_1 \leq  C\left(\frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2}\right), \qquad \forall \la \in (0,\la_0),
$$
and the conclusion follows.


Otherwise, let $t_1$ and $t_2$ be respectively the smallest  and largest values of $ t\in [s_1,s_2]$ for which   $\Hh^1(\partial^M E_t \cap T_{r/2} )>0$. 

We can now show that $\Hh^1(\partial^* F_t \cap T_{r/2} )>0$ for all $t\in [t_1,t_2]$:  Let $t\in (t_1,t_2)$. Let $x_1\in \partial^M E_{t_1} \cap T_{r/2}$ and $x_2\in \partial^M E_{t_2}\cap T_{r/2}$. Suppose that $\Hh^1(\partial^M E_t \cap T_{r/2})=0$. Then, since $x_2\in E_{t_2}\subset E_{t}$, we must have $x_2\in \mathring{E_{t}}$. If $x_1\in E_t$, then we must have $x_1\in \partial^M E_t$ since $E_t\subset E_{t_1}$, but since $\partial^M E_t \cap T_{r/2}=\emptyset$, this is impossible. So, $x_1\not\in E_t$. We can now define a continuous curve $\gamma:[a,b]\to T_{r/2}$ with $\gamma(a) = x_1$ and $\gamma(b) = x_2$. However, because $x_1\not\in E_t$, $x_2 \in \mathring{E_t}$, $\gamma$ must intersect $\partial^M E_t$, which contradicts our assumption that $\partial^M E_t \cap T_{r/2}=\emptyset$.  Thus, $0<\Hh^1(\partial^M E_{t} \cap T_{r/2}) =  \Hh^1(\partial^* F_{t} \cap T_{r/2}) $ for all $t\in [t_1,t_2]$.



So, by Proposition \ref{prop:closed_curves_viaBurger} and Theorem \ref{thm:burger_outside_tube},  
\begin{equation}\label{eq:osc_bd1}
 t_2 - t_1 \leq \frac{2}{r(1-e_{r/2})}\left(\frac{\delta^2}{2\lambda } +\frac{\lambda  \norm{v}_{L^2}^2}{2 } + \delta \norm{v}_{L^2} \right),
\end{equation}
and since $F_s\subset T_{r/2}$ for all $s \in [s_1,t_1)\cup (t_2,s_2]$,
\begin{equation}\label{eq:osc_bd2}
 s_2-t_2+s_1-t_1 \leq C \left(\frac{\delta^2}{2\lambda} +\frac{\lambda  \norm{v}_{L^2}^2}{2} + \delta \norm{v}_{L^2}\right)
\end{equation}
for all $\la$ sufficiently small.
The result follows by adding together (\ref{eq:osc_bd1}) and (\ref{eq:osc_bd2}).
\end{proof}

\begin{prop}\label{prop:curvature_viaBurger}
 There exists $C>0$ and $\la_0>0$ such that the following holds:
  Let $s_1,s_2\in \RR$ and let $F_t = \{ u_\lambda > t\}$. If $\Hh^1(\partial^* F_t \cap T_r) = 0$ for all $t\in [s_1,s_2]$, then 
$$C(s_2-s_1)  \leq  \int_{T_r^c}\abs{D u_\la}.
$$
\end{prop}
\begin{proof}
By Lemma \ref{lem:lower_bound_lev_sets}, there exists $\la_0$ and $C>0$ such that if $\la\leq \la_0$ and $P(F_t)\neq 0$, then $P(F_t)\geq C$. Therefore, by the co-area formula,
$$C(s_2-s_1) \leq \int_{t=s_1}^{s_2} P(F_t)\mathrm{d}t \leq  \int_{T_r^c}\abs{D u_\la}.
$$

\end{proof}

\begin{prop}\label{prop:closed_curves_viaBurger}
 Let $F_t = \{ u_\lambda > t\}$ and suppose that $\Hh^1(\partial^* F_t \cap T_{2r}^c)\neq 0$ and $\Hh^1(\partial^* F_t \cap T_{r})\neq 0$ for all $t\in [s_1,s_2]$. Then,
 $$
 s_2-s_1 \leq \frac{1}{r }\int_{T_r^c}\abs{D u_\lambda} 
$$
\end{prop}
\begin{proof}
 By our assumption on the level sets $F_t$ and since $\partial^M F_t$ is continuous, for each $t\in [s_1,s_2]$,   there exists $x_1\in T_{r}$ and $x_2\in T_{2r}^c$ such that $\gamma(a)  = x_1$ and $\gamma_{\lambda}(b) = x_2$ where $\gamma_\lambda : [a,b] \to \Omega$ is continuous and $\gamma_\lambda \subset \partial^M F_t\setminus T_{r}$. Note that the length of $\gamma$ is at least $r$ and so, $P(F_t, T_r^c)= \Hh^1(\partial^M F_t \setminus T_r) \geq r$. By the co-area formula,
$$
\int_{T_r^c}\abs{D u_\lambda} \geq \int_{s_1}^{s_2} P(F_t; T_r^c) \mathrm{d}t \geq (s_2-s_1)r.
$$ 

\end{proof}

==> sections/sec-calibrable-rn.tex <==
% !TEX root = ../TV-Denoising.tex

% THIS FILE IS DEPRECATED: IT IS INCORPORATED IN PRELIMINARIES

\subsection{Calibrable sets in $\RR^N$}
\todo{Put this section inside the preliminaries}

\subsubsection{Sets that evolve at constant speed}
In \cite{beltvflow02}, the authors study on the total variation flow $\frac{\partial u}{\partial t}\in -\partial J(u)$, namely:
\begin{align}
  \frac{\partial u}{\partial t}= \divx \left(\frac{Du}{|Du|} \right).
  \label{eq-tvflow}
\end{align}
The prove existence and uniqueness of a ``strong solution" (see \cite{beltvflow02}) for all initial data $u_0\in \LDN$, and existence and uniqueness of an ``entropy solution" for $u_0\in L^1_{loc}(\RR^N)$.
In the second part of the paper, they characterize the bounded sets of finite perimeter $\Omega$ such that $u=\bun{\Omega}$ satisfies
\begin{align}
  -\divx \left(\frac{Du}{|Du|}\right)= \lambda_\Omega u, \quad \mbox{ where } \la_\Omega\eqdef \frac{P(\Omega)}{|\Omega|}.
\end{align}

Let us show (at least informally) that such sets are exactly the sets which evolve with constant boundary, i.e. such that $u(x,t)=\la(t)\bun{\Omega}(x)$, with $\la \geq 0$.
On the one hand $\frac{\partial u}{\partial t}= \la'(t)\bun{\Omega}$, and on the other one, $\divx \left(\frac{Du}{|Du|}\right)=\divx\left(\frac{D\bun{\Omega}}{|D\bun{\Omega}|} \right) $ for $\la(t)>0$, so that \eqref{eq-tvflow} is equivalent to
\begin{align*}
  -\la'(t)\bun{\Omega}= \divx \left(\frac{D\bun{\Omega}}{|D\bun{\Omega}|}\right),
\end{align*}
hence, integrating over $\Omega$, we get 
\begin{align*}
  -\la'(t) |\Omega|=\int_\Omega \divx\left(\frac{D\bun{\Omega}}{|D\bun{\Omega}|} \right)=\int_{\partial^* \Omega} \frac{D\bun{\Omega}}{|D\bun{\Omega}|}\cdot \nu_{\Omega}d\Hh^1=P(\Omega).
\end{align*}
As a consequence $\la(t)=(1-\la_\Omega t)_+$.


Such sets are called calibrable. They are characterized by the fact that $\la_\Omega\bun{\Omega}\in \partial J(\bun{\Omega})$:

\begin{defn}[Calibrable sets]
  A set of finite perimeter $\Omega\subset \RR^N$ is said to be calibrable if, writing $v=\bun{\Omega}$, there exists a vector field $\xi\in L^{\infty}(\RR^N,\RR^N)$ such that $\|\xi\|_\infty \leq 1$
  and 
  \begin{align}
    \int_{\RR^N} (\xi, Dv)=\int_{\RR^2} |Dv|,\\
    -\divx \xi =\la_\Omega v.
  \end{align}
  In that case, we say that $\xi$ is a calibration for $\Omega$.
\end{defn}

\begin{rem} If $\la \bun{\Omega}\in \partial J(\bun{\Omega})$ for some $\la\in \RR$, then necessarily $\la=\la_\Omega$.
\end{rem}


\subsubsection{Inner and outer calibrations}
\vd{The notion of inner and outer calibrations is used in~\cite{beltvflow02} to construct calibrations "inside" and "outside" the studied sets. It is defined in $\RR^2$ but I guess everything works in $\RR^N$..}

\begin{defn}
Let $\Omega \subseteq \RR^2$ be a set of finite perimeter. We say that $\Omega$ is $-$calibrable if there exists a vector field $\xi^-_\Omega: \RR^2\rightarrow \RR^2$ 
such that 
\begin{enumerate}
  \item $\xi^-_\Omega\in L^2_{loc}(\RR^2,\RR^2)$ and $\divx \xi^-_\Omega \in L^2_{loc}(\RR^2)$;
  \item $|\xi^-_{\Omega}| \leq 1$ almost everywhere in $\Omega$;
  \item $\divx \xi^-_\Omega$ is constant on $\Omega$;
  \item $\theta(\xi^-,-D\bun{\Omega})(x)=-1$ for $\Hh^1$-almost every $x\in \partial \Omega^*$.
\end{enumerate}
Similarly $\Omega$ is $+$calibrable if $1),2),3)$ hold and $\theta(\xi^+,-D\bun{\Omega})(x)=+1$ in $4)$.
\end{defn}
The following lemma tells that one may "glue" calibrations:
\begin{lem}[\protect{\cite{beltvflow02}}]
  Let  $\Omega$ be a bounded set of finite perimeter. Then $v=\bun{\Omega}$ is calibrable if and only if $\Omega$ is $-$calibrable with $-\divx \xi^-_{\Omega}=\la_\Omega$ in $\Omega$, and $\RR^2\setminus \Omega$ is $+$calibrable with $\divx \xi^+_{\RR^2}=0$ in $\RR^2\setminus \Omega$,
  defining
  \begin{align*}
    \xi:= \left\{ \begin{array}{cc}
        \xi^-_\Omega & \mbox{on }  \Omega,\\
        \xi^+_\Omega & \mbox{on } \RR^2\setminus \Omega.
    \end{array}\right.
  \end{align*}
\end{lem}



\subsubsection{Characterization in $\RR^2$}

\begin{prop}[\protect{\cite{beltvflow02}}]
Let $C\subset \RR^2$ be a bounded set of finite perimeter, and assume that $C$ is connected. $C$ is calibrable if and only if the following three conditions hold:
\begin{enumerate}
  \item $C$ is convex;
  \item $\partial C$ is of class $C^{1,1}$;
  \item the following inequality holds:
    \begin{align}
      \ess \sup_{p\in \partial C} \kappa_{\partial C} (p)\leq \frac{P(C)}{|C|}.
    \end{align}
\end{enumerate}
\end{prop}
\begin{prop}[\protect{\cite{beltvflow02}}]
Let $\Omega \subset \RR^2$ be a bounded set of finite perimeter which is calibrable. Then,
\begin{enumerate}
  \item The following relation holds:
    \begin{align}
      \frac{P(\Omega)}{|\Omega|} \leq \frac{P(D)}{|D\cap \Omega|}, \quad \forall D\subseteq \RR^2, D \mbox{ of finite perimeter;}
    \end{align}
  \item each connected component of $\Omega$ is convex.
\end{enumerate}
\end{prop}


==> sections/sec-stability-grad.tex <==
% !TEX root = ../TV-Denoising.tex

\section{Stability of the support of the gradient}\label{sec:stab_grad}
\todo{The previous section shows that one has support stabiliy ouside the extended support. This section shows that if we knew the behaviour of $z_0$, then we can have more precise bounds on the support stability regions. }


Let $f\in \LDD \cap \BVD$ such that \eqref{eq-constr-dual} has a solution (source condition). 
Let $v_0$ be the corresponding minimal norm certificate.

We define a tube around the extended support
\begin{equation}
  T_r\eqdef \enscond{x\in \RR^2}{\mathrm{dist}(x,\ext(Df))\leq r }
\end{equation}

We assume that (see for instance Section~\ref{sec:calibrable} for examples),

\begin{equation*}
  \deltar\eqdef 1-\ess \sup_{x\in T_r^C} \abs{z_0(x)}>0.\label{eq:defer}
\end{equation*}
\todo{finish to incorporate the noise in this section}
Let $E_\la$ be any level set of the solution $\ulaw$ of~$(\Pp_\la(f+w))$ . We assume without loss of generality that $\abs{E_\la}<+\infty$. We denote by $\vlaw$ (resp. $\vla$) the solution of $(\Dd_\la(f+w))$ (resp. $\Dd_\la(f))$)

 


\begin{prop}\label{prop:partoutsidetube}
  There is a constant $C>0$ (which only depends on $v_0$) such that 
\begin{equation}
  \deltar \HDU{\partial^*E_{\la,w}\setminus T_r}\leq \int_{E_{\la,w}}(v_{\la,w} - v_0)\leq C\normLdeux{v_{\la,w}-v_0},
\end{equation}
\end{prop}


\begin{proof}
Comparing the energy of $E_{\la,w}$ with that of the empty set we get,
\begin{align*}
  P(E_{\la,w})\leq \int_{E_{\la,w}}v_{\la,w} &= \int_{E_{\la,w}}(v_{\la,w}-v_0) + \int_{E_{\la,w}}v_0
  \\
                                 &\leq \normLdeux{v_{\la,w}-v_0}\sqrt{\abs{E_{\la,w}}} + \int_{\partial^* E_{\la,w}} z_0\cdot \nu
                                 \\
  \mbox{hence }  P(E_{\la,w})- \int_{\partial^* E_{\la,w}\cap T_R}z_0\cdot \nu - \int_{\partial^* E_{\la,w}\setminus T_r}z_0\cdot \nu &\leq C \normLdeux{v_{\la,w}-v_0}.
\end{align*}
Since $\left(\ess \sup_{\RR^N\setminus T_r}\abs{z_0}\right)\leq 1-\deltar$, and more generally $\normLinf{z_0}\leq 1$, 
\begin{align*}
  P(E_{\la,w})- \int_{\partial^* E_{\la,w}\cap T_R}z_0\cdot \nu - \int_{\partial^* E_{\la,w}\setminus T_r}z_0\cdot \nu  &\geq \HDU{\partial^*E_{\la,w}\setminus T_r}+\HDU{\partial^*E_{\la,w}\cap T_r}\\
                                                                                                            &- (1-\deltar)\HDU{\partial^*E_{\la,w}\setminus T_r} - \HDU{\partial^*E_{\la,w}\cap T_r}\\
                                                                                                            &\geq  \deltar \left(\HDU{\partial^*E_{\la,w}\setminus T_r}\right),
\end{align*}
hence the claimed result.

\end{proof}



\begin{prop}\label{prop:entiretubecomplement}
Let $\la>0$ and $w\in \LDD$ be such that $\normLdeux{v_{\la,w}-v_0} <2\sqrt{\pi}\deltard$. Then, $E\in \FFlaw$ and $P(E)>0$ implies that
  \begin{equation}
    \HDU{\partial^* E \cap T_{r/2}}>0.
  \end{equation}
\end{prop}
\begin{proof}
Assume by contradiction that $P(E)>0$ and $\HDU{\partial^* E\cap T_{r/2}}=0$ so that $\partial^* E \subset T_{r/2}^c$ up to an $\Hh^1$-negligible set. Then,
\begin{align*}
P(E) &= \int_E \vlaw \leq \norm{E}^{1/2} \normLdeux{\vlaw - \voo} + \int_E \voo\\
&\leq \frac{P(E) \normLdeux{\vlaw - \voo} }{2\sqrt{\pi}}+ (1-\delta_{r/2}) P(E)
\end{align*}
where we have applied the isoperimetric inequality and the fact that $\voo = \divx z_0$ with $\abs{z_0}leq (1-\delta_{r/2})$ on $T_{r/2}^c$. Since $P(E)>0$, this implies that
$$
2\delta_{r/2}\sqrt{\pi} \leq \normLdeux{\vlaw - \voo}.$$
This contradicts the assumption of this proposition.
\end{proof}



We obtain the following stability theorem in the case $N=2$.


\begin{thm}
 If $\la>0$ and $w\in \LDD$ are such that
  $$
  \norm{v_{\la,w} - v_0}_{L^2}\leq \frac{r\delta_{r/2}}{2},
  $$
  then
up to an $\Hh^1$-negligible set,
\begin{equation}
  \partial^* E_{\la,w} \subseteq T_r.
\end{equation}

\end{thm}


